The convex core of quasifuchsian manifolds with particles

We consider quasifuchsian manifolds with "particles", i.e., cone singularities of fixed angle less than $\pi$ going from one connected component of the boundary at infinity to the other. Each connected component of the boundary at infinity is then endowed with a conformal structure marked by the endpoints of the particles. We prove that this defines a homeomorphism from the space of quasifuchsian metrics with $n$ particles (of fixed angle) and the product of two copies of the Teichm\"uller space of a surface with $n$ marked points. This is analoguous to the Bers theorem in the non-singular case. Quasifuchsian manifolds with particles also have a convex core. Its boundary has a hyperbolic induced metric, with cone singularities at the intersection with the particles, and is pleated along a measured geodesic lamination. We prove that any two hyperbolic metrics with cone singularities (of prescribed angle) can be obtained, and also that any two measured bending laminations, satisfying some obviously necessary conditions, can be obtained, as in [BO] in the non-singular case.

==> conebend36.tex <==
\subsection{The bending lamination of the convex core}

To finish the proof of Lemma \ref{lm:compact} we only have to check that
the induced bending lamination on the boundary of the convex core of the
limit manifold is the limit of the bending laminations. We can state
the result as follows.

\begin{lemma} \label{lm:limit-bending}
Let $N=S\times I$, let $p_1,\cdots, p_m$ be distincts points on $S$, and let  
$\kappa_i=\{ p_i\}\times I, 1\leq i \leq m$. 
Let $(g_n)_{n\in \N}$ be a sequence of quasifuchsian metrics on $N$ with a particle
of angles $\theta^i_n$ along $\kappa_i$, $1\leq i\leq m$. 
Let $\lambda_n$ be the measured bending 
laminations on the boundary of the convex core of $N$ (considered 
as a measured lamination on $\dr N$ minus the endpoints of the $\kappa_i$), and 
let $m_n$ be the induced metric on the boundary of $N$. 
Suppose that $(g_n)$ converges in bilipschitz topology towards a quasifuchsian
metric with particles $g$, with cone angles $\theta^i\in (0,\pi)$ along $\kappa_i$.
Then $(m_n)_{n\in \N}$ converges to the induced metric $m$ on the boundary of the convex core
in $(N,g)$, while $(\lambda_n)_{n\in \N}$ converges to the measured bending lamination
$\lambda$ of the boundary of the convex core of $(N,g)$. 
\end{lemma}

\begin{proof}
Let $(\gamma_n)_{n\in \N}$ be a sequence of segments in $N$, with $\gamma_n$
geodesic for $g_n$ for all $n\in \N$. 
Suppose that $(\gamma_n)_{n\in \N}$ converges to a segment $\gamma$.
Since $g_n\rightarrow g$ in the bilipschitz topology and, in hyperbolic geometry,
any segment which is close to realizing the distance between its endpoints is close 
to a geodesic segment. So $\gamma$ is geodesic for $g$. Conversely, any geodesic
segment for $g$ is a limit of geodesic segments for the $g_n$. The same holds for
closed geodesics.

Let $(\Omega_n)_{n\in \N}$ be a sequence of compact subsets of $N$ such that, for all 
$n\in \N$, $\Omega_n$ is convex for $g_n$. Suppose that $\Omega_n\rightarrow \Omega$
in the Hausdorff topology. 
The definition of a convex subset and the previous paragraph show that $\Omega$ 
is convex, since any geodesic segment $\gamma$ in $(N,g)$ with endpoints in 
the interior of $\Omega$ is
the limit of a sequence of geodesic segments $\gamma_n$, with $\gamma_n$ geodesic for
$g_n$. Since $\gamma_n$ has endpoints in $\Omega_n$ (for $n$ large enough) and 
$\Omega_n$ is convex for $g_n$, $\gamma_n\subset\Omega_n$, and therefore 
$\gamma\subset \Omega$, and $\Omega$ is convex for $g$. 
Conversely, a similar argument shows that any compact convex subset for $g$ is the 
Hausdorff limit of a sequence of compact convex subsets of the metrics $g_n$.

For all $n$, $\convn$ contains all closed geodesics in $(N, g_n)$. Given a 
non-trivial homotopy class $\alpha$ in $N_r$ (the complement of the singular curves 
in $N$), it is realized for each $n\in \N$ by a (unique) closed geodesic $\gamma_n$ in 
$(N,g_n)$, and the sequence $(\gamma_n)_{n\in \N}$ converges to the closed geodesic $\gamma$
which realizes $\alpha$ in $(N,g)$. For each $n\in \N$, $\gamma_n\subset \convn$.
Moreover we have seen that the diameter of the $\convn$ is bounded. It follows that
$(\conv_n)_{n\in \N}$ converges -- after extracting a subsequence -- to a limit 
subset $C'$ which contains all closed geodesics in $(N,g)$. 

Since $C'$ is the limit of a sequence of convex subset of the $(N,g_n)$, it is
convex. Moreover
if $\Omega\subset C'$ is convex, then it is the limit of a sequence of convex 
subsets $\Omega_n\subset \convn$. But then $(\Omega_n\cap \convn)_{n\in \N}$ 
is a sequence of convex subsets converging to $\Omega$. Because the $\convn$
are minimal convex subsets, $\Omega_n\cap \convn=\convn$ for all $n$, so 
that $\Omega=C'$. So $C'=\conv$. This shows that $\conv$ is the Hausdorff
limit of the $\convn$. 

Note that it is not clear at this point whether $\partial\convn\rightarrow \partial \conv$
in the $C^1$ topology. However the $C^0$ convergence (together with the bilipschitz convergence
of $g_n$ to $g$) is sufficient to insure that the metric $m_n$ on $\dr \convn$
is {\it larger} in the limit than the metric by $g$ on $\dr \conv$. In other terms,
if $x,y\in \dr \conv$ and $x_n,y_n\in \dr \convn$ are such that $\lim x_n=x, \lim y_n=y$,
then there exists for each $\epsilon>0$ some $n\in \N$ such that, for 
all $n\geq N$, 
$$ d_{m_n}(x_n,y_n)\geq (1-\epsilon)d_m(x,y)~. $$
It follows that the lengths of the closed geodesics in $S$ for $m_n$ are 
bounded from below by $(1-\epsilon)$ times their lengths for $m$. 

Since the metrics $m_n$ and $m$ are hyperbolic metrics with cone singularities of 
fixed angles, this shows, using standards arguments based for instance on pants
decompositions, that $m_n\rightarrow m$ (see \cite{dryden-parlier}).

It then follows that as $n\rightarrow \infty$, $m_n$ is bounded from above by
$(1+\epsilon)m$: under the same hypothesis as above, 
$$ d_{m_n}(x_n,y_n)\leq (1+\epsilon)d_m(x,y)~. $$
Since $m_n\rightarrow m$ in this sense, and moreover $\dr\convn\rightarrow \dr \conv$
in the $C^0$ topology, it follows that the measured bending laminations on 
$\dr \convn$ converges to the measured bending lamination on $\dr\conv$, 
$\lambda_n\rightarrow \lambda$.
\end{proof}

